Trapping Single Ions and Coulomb Crystals with Light Fields

The scope of this book is on providing insight into the recently emerged field of optical trapping of ions. Since the ground-breaking introduction of light fields as tools for exerting trapping forces on matter in 1970 by Ashkin, optical dipole traps have enabled an unprecedented level of control over neutral atoms and molecules both at the level of quantum ensembles as well as individual particles. It was found recently that in some situations it is highly advantageous to confine atomic and molecular ions without employing any radiofrequency-based Paul traps or strong external magnetic fields as used in Penning traps, e.g. when investigating the interaction of neutral atoms and ions in the regime of ultralow interaction energies. Adapting optical traps for ions is a promising way to approach such scenarios and the focus of this work is to present a comprehensive overview of the background and concepts behind this technique as well as to discuss the currently achievable level of control, encountered limitations and perspectives for future applications.

==> TeX_files/chapter06.tex <==
\chapter{Introduction - 2} \label{chpt:Intro-2}

Over the past decades, optical forces have proved to be a pivotal instrument for confinement and manipulation of atoms \cite{Phillips1998,Chu1998,Cohen-Tannoudji1998}. Their use has enabled highly versatile trap geometries while at the same time preserving the capability to investigate interactions of atomic gases and molecules at ultralow temperatures \cite{Bloch2008}.
% allows for ensembles of neutral atoms allows for highly versatile trap geometries while at the same time preserving the capability to investigate interactions of atomic gases and molecules at ultralow temperatures \cite{Bloch2008}.
Optical traps are now routinely used to trap and control individual neutral atoms and atomic ensembles on the nanoscale with sub-wavelength resolution, e.g. in the Mott insulator regime \cite{Bloch2005} or in the demonstrated realizations of quantum gas microscopes \cite{Bakr2009,Sherson2010} (Fig. \ref{fig:QuantGasMikroscope}). Recently these techniques have been once more tremendously improved by refining the control over combinations of several optical fields and making use of the available degrees of freedom such as geometry, intensity, polarizations and relative phases \cite{Greif2015,Morsch2006,Bloch2008}. Consequently, this progress has led to the realization of superlattices \cite{Kangara2018}, and Kagom\'{e} lattices \cite{Jo2012} (Fig. \ref{fig:OptLattice}), as well as to the assembly of linear \cite{Endres2016}, two-dimensional \cite{Barredo2016} and even three-dimensional arrays \cite{Barredo2018} of atoms.\\

\makeatletter
\@addtoreset{footnote}{section}
\makeatother

\begin{figure}[h!]
	\subfigure[]{
		\includegraphics[width=0.3\textwidth]{figure1_1_a.pdf}
		\label{fig:QuantGasMikroscope}
	}
	%%%
	\subfigure[]{
		\includegraphics[width=0.7\textwidth]{figure1_1_b.pdf}
		\label{fig:OptLattice}
	}
	\caption[]{Optical trapping potentials in experiments with neutral atoms: \textbf{(a)} individual  atoms imaged within the optical potential of a standing wave (courtesy of W. Bakr, taken from \cite{Bakr2009}) and \textbf{(b)} versatile optical trapping  geometries (from left to right: triangular, polarization, and honeycomb lattice) obtained by using a superposition of three laser beams and controlling their respective polarizations (courtesy of K. Sengstock, taken from \cite{Luehmann2014})\footnotemark[1] .}
	 %\cite{Becker2010}
\end{figure}


%\footnote{Reprinted figure with permission from . Physical Review A, 90:013614 (2014). Copyright (2019) by the American Physical Society.}
%Dirk-S\"{o}ren L\"{u}hmann, Ole J\"{u}rgensen, Malte Weinberg, Juliette Simonet,	Parvis Soltan-Panahi, and Klaus Sengstock

For several decades, the exquisite degree of control over individual atoms has been one of most prominent characteristic features in the field of ion trapping, a vastly successful and rapidly expanding area of atomic physics \cite{Paul1990,Wineland2013}.
In this field of research, individual atoms are typically confined in radiofrequency or Penning traps, affording preparation, operation and detection fidelities approaching unity and storage times on the order of months or years. 
%
Motional and internal electronic degrees of freedom of atomic ions can be manipulated on the quantum level with individual addressability and exceptionally high operation fidelities in excess of 99$\%$ \cite{Monroe2013,Gaebler2016,Ballance2016}, making trapped ions one of the most promising and performant platforms for quantum information processing (QIP), quantum simulations and metrology to date. Long-range interactions that are difficult to establish in experiments with neutral atoms allow for using phonon modes of Coulomb crystals as a bus for generating entanglement between ions in linear chains \cite{Blatt2012}.\\

\begin{figure}
	\subfigure[]{
	\includegraphics[height=0.3\textwidth]{figure1_2_a.pdf}
				}
			\label{fig:PaulTrapPicture}
	\hspace{.05\textwidth}
	\subfigure[]{
	\includegraphics[height=0.3\textwidth]{figure1_2_b.pdf}
%	\includegraphics[height=0.3\textwidth]{3d_ion_crystal.pdf}
				}
			\label{fig:IonCrystalPicture}
	\caption{\textbf{(a)} Linear Paul trap with segmented electrodes. The diagonal spacing between the electrodes is $ 18 \, mm $. \textbf{(b)} False-color fluorescence image of a three-dimensional ion Coulomb crystal. The spacing between the ions is determined by the choice of the trap parameters. Typically, the ions are separated by approximately $ 20 \, \mu m $ allowing for individual addressability.}
	\label{fig:PaulTrapAndIons}
\end{figure}
% copy right note: (adapted from \cite{Schneider2012b})?

\footnotetext[1]{Reprinted figure with permission from D.-S. L\"{u}hmann, O. J\"{u}rgensen, M. Weinberg, J. Simonet,	P. Soltan-Panahi, and K. Sengstock. Physical Review A, 90:013614 (2014). Copyright 2019 by the American Physical Society.}

While Paul traps have proved to be very successful or leading platforms for applications in many fields of contemporary research, some outstanding challenges closely related to limitations in scalability have emerged. The generation of nanoscale potentials with Paul traps remains another challenge despite of rapid advances achieved with planar trapping geometries. An intrinsic property of such radiofrequency (rf) traps is the driven motion at the modulation frequency which is superimposed with the secular motion of ions as illustrated in figure \ref{fig:MuMotion}. While this so-called micromotion can be neglected in most applications based on the manipulation of common mode excitations within linear ion crystals, it can impose a fundamental limitation on other experiments sensitive to kinetic energy \cite{Cetina2012,Tomza2017}. A prominent example is the rapidly growing field of ion-atom interactions \cite{Grier2009,Schmid2010,Zipkes2011a,Meir2016,Kleinbach2018,Fuerst2018,Dutta2017,Haze2018} where the presence of driven electromagnetic fields typically limits the accessible collision energies to the range of 1 mK \cite{Haerter2014,Tomza2017}. While some approaches exploiting the favorable kinematic properties of specific combinations of neutral atom and atomic ion species confined in conventional Paul traps exist \cite{Cetina2012,Fuerst2018} and seem promising for accessing a range of collision energies that could approach the quantum interaction regime, the generalization to either generic atom-ion combinations or to experiments involving more than a single ion or a linear chain remains an outstanding challenge in the field and stands to benefit from alternative ways to avoid micromotion. One recently demonstrated approach along these lines relies on the preparation of highly excited Rydberg states within a Bose-Einstein-Condensate, which then behave as ions immersed in an atomic bath \cite{Kleinbach2018}. So far the achieved kinetic energies of the Rydberg atoms correspond to temperatures on the order of microkelvin, and the sensitivity of the system to stray electric fields as well as the comparably short lifetime of the Rydberg excitations remain challenging.\\

\begin{figure}
	\begin{center}
		\includegraphics[height=0.4\textwidth]{figure1_3.pdf}
		%\includegraphics<2>[height=0.5\textwidth]{MOTandIons.pdf}
		%	{$ E_{col} $ limited by micromotion-induced heating $\rightarrow$ fundamental in all rf traps}
	\end{center} 
\caption{Motion of an ion in a radiofrequency trap. The oscillation at a frequency $ \omega_{sec} $ in the quasi-harmonic trapping potential is superimposed with a rapid oscillation at the modulation frequency of the trap, $ \Omega_{rf}$. In the presence of any stray electric field the amplitude of this micromotion is non-zero at all times (upper trace).}
	\label{fig:MuMotion}	
\end{figure}

In view of these considerations, a naturally seeming approach for addressing the issues highlighted above would be to use the powerful set of tools and methods provided by optical potentials and combine it with the advantaged granted by ions and Coulomb crystals as a platform for experimental investigations. The recently emerged field of optical traps for ions aims at harvesting exactly the potential of this synergetic combination \cite{Schaetz2017}. Dynamically applied optical forces are instrumental in quantum information processing with ions \cite{Wineland2013,Leibfried2003} as a route towards mediating state-dependent interactions \cite{Monroe1995,Blatt2012,Friedenauer2008,Blatt2008}. Static optical potentials have been used to study anomalous ion diffusion \cite{Katori1997}. Despite the broad use of optical forces and potentials for the manipulation of ions, it was only in 2010 that they have been successfully used to demonstrate optical trapping of a single ion \cite{Schneider2010} in absence of any rf fields. Since then the employed techniques and methods have undergone a continuous development in terms of performance and feasibility culminating in a series of experiments \cite{Schneider2012,Schneider2012b,Enderlein2012,Huber2014,Lambrecht2017,Schaetz2017,Schmidt2018}. These investigations will be in the focus of the following discussion aiming  to provide a dissemination of the basic concepts behind this approach as well as its applicability to the outstanding experimental issues outlined in the previous paragraphs.\\

Another closely related class of experiments is based on a combination of radiofrequency traps with optical standing waves \cite{Linnet2012,Karpa2013,Laupretre2019}. This approach provides composite trapping potentials with wavelength-scale periodicity whose implementation in conventional, purely rf-driven, traps including planar chip technology, to this day remains a highly demanding task exceeding the state-of-the-art.
%
It is worth pointing out that combining several established trapping techniques in order to obtain a system with a unique set of advantageous properties has been a very successful strategy in the past. For example, a combination of linear Paul traps and Penning traps allows for a suppression of the magnetron frequency and can lead to an improved performance of mass spectrometers \cite{Huang1997}.
%
In the more recent case, the obtained nanoscale corrugation of the effective potential in one dimension is the unique feature of the hybrid setups mentioned above. They turned out to be a nearly ideal platform for investigating theoretically treated phenomena such as structural transitions of one-dimensional ion chains \cite{Pruttivarasin2011,Benassi2011} and have recently lead to the first realization of friction models on the level of a few atoms \cite{Bylinskii2015,Gangloff2015}. Although in this hybrid trapping approach the presence of micromotion still hinders the straightforward extension to higher dimensional systems, in the future, radiofrequency-free trapping potentials realized in optical traps could open up a novel field of studies shedding light on structural phase transitions between one, two and three dimensional ordering close to a quantum critical point \cite{Baltrusch2011,Baltrusch2012,Shimshoni2011,Shimshoni2011a}. This however requires the capability to prepare such higher-dimensional Coulomb crystals in the quantum regime which is another outstanding challenge in contemporary atomic physics.\\

On a similar note, the availability of quasi-static and state-dependent potentials confining 2d ion crystals could also provide a platform for novel quantum simulations \cite{Schneider2012b,Zoller2000}, e.g. the study of fracton models \cite{Pretko2018} or contribute to the field of quantum information processing by utilizing the state-dependent nature of optical potentials to realize fast gate operations as an alternative to approaches based on Rydberg ions \cite{Feldker2015,Higgins2017,Higgins2017a} or fast Raman transitions \cite{Campbell2010}. Lastly, ions in optical potentials may be a used as a nanoscale probe with implications in the field of metrology and sensing of ambient fields. \\

The aim of the following sections is to present an overview of the recent advances in the field of optical trapping of ions and Coulomb crystals as well as to provide a detailed description of the prerequisites, experimental techniques, limitations and prospects of this approach for such envisioned applications.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliographystyle{unsrtnat}

\bibliography{chapter01}

\chapter*{Acknowledgments}

The projects described in this work have received funding from the European Research Council (ERC) under the European Union’s Horizon 2020 research and innovation program (Grant No. 648330). The author is grateful for financial support from the Alexander von Humboldt Foundation and Marie Curie Actions.\\

I am indebted to all my colleagues who have contributed to several generations of optical trapping experiments. In particular, it was my privilege to work side by side with T. Huber, J. Schmidt, A. Lambrecht, and of course, T. Schätz who has conceived and initiated the experiments on optical ion trapping. I would especially like to thank Vladan Vuleti\'{c} for introducing me to the field, our numerous fruitful discussions, as well as his prudent advice and support.\\

==> TeX_files/preface.tex <==
%
\chapter*{Preface}

The scope of this book is on providing insight into the recently emerged field of optical trapping of ions. Ever since the ground-breaking introduction of light fields as tools for exerting trapping forces on matter in 1970 by Arthur Ashkin \cite{Ashkin1970}, optical dipole traps have been used with remarkable success in several fields of research, most notably in atomic physics, where they have enabled an unprecedented level of control over neutral atoms and molecules both at the level of quantum ensembles\cite{Bloch2008} as well as individual particles \cite{Endres2016,Barredo2018}.\\

Another tremendously influential development in Physics was enabled by the invention of radiofrequency traps pioneered by Paul \cite{Paul1990} and Dehmelt, allowing for confinement of single atomic ions demonstrated by Wineland \cite{Wineland2013} decades before this was realized on the level of individual neutral atoms in optical traps. Ions provide a number of properties that render them ideal for state-of-the-art applications in several cutting-edge areas of contemporary research ranging from metrology \cite{Rosenband2008}, quantum simulation and computation \cite{Blatt2008} to ultracold chemistry \cite{Cote2002}.\\

However, it was found recently that in some situations it is highly advantageous to confine ions without employing any radiofrequency-based Paul traps or strong external magnetic fields in Penning traps, e.g. when investigating the interaction of neutral atoms and ions in the regime of ultralow interaction energies \cite{Haerter2014}. Adapting optical traps for ions \cite{Schaetz2017} is a promising way to approach such scenarios and the focus of this work is to present a comprehensive overview of the background and concepts behind this technique as well as to discuss the currently achievable level of control, encountered limitations and perspectives for future applications.\\

\newpage
Chapter 1 is intended to provide a context of the described experiments within the field of atomic physics. It highlights the advantages of the currently used techniques applied for trapping and manipulating ions in comparison with the features granted by optical traps for neutral atoms. \\

Chapter 2 lays out the general concepts, requirements and methodology for realizations of optical trapping of ions.\\

Chapter 3 describes how the tools and methods presented in the previous chapter can be used to confine single atomic ions in optical traps. Individual developments achieved in the last years are highlighted by presenting and discussing milestone experiments \cite{Schneider2010,Enderlein2012,Huber2014,Lambrecht2017}. The aim of this chapter is to provide an understanding of the current performance granted by this approach and its prospective possibilities for applications in the near future. It concludes with a discussion of the identified limitations and strategies for future improvement.\\

Chapter 4 is focused on experiments reaching beyond the established optical traps for single ions. It provides an in-depth view on the recently demonstrated extension of the presented methods to the case of ion Coulomb crystals \cite{Schmidt2018}.\\

Chapter 5 highlights the key features of the concepts discussed in this book, summarizes the main features of optical traps for ions and provides an outlook for future applications building on the capabilities afforded by these novel tools.\\

\begin{flushright}
Leon Karpa
\end{flushright}

\newpage
\chapter*{Dedication}
This work is dedicated to my family.
